On Tuza's Conjecture in Dense Graphs

In 1982, Tuza conjectured that the size $\tau(G)$ of a minimum set of edges that intersects every triangle of a graph $G$ is at most twice the size $\nu(G)$ of a maximum set of edge-disjoint triangles of $G$. This conjecture was proved for several graph classes. In this paper, we present three results regarding Tuza's Conjecture for dense graphs. By using a probabilistic argument, Tuza proved its conjecture for graphs on $n$ vertices with minimum degree at least $\frac{7n}{8}$. We extend this technique to show that Tuza's conjecture is valid for split graphs with minimum degree at least $\frac{3n}{5}$; and that $\tau(G) < \frac{28}{15}\nu(G)$ for every tripartite graph with minimum degree more than $\frac{33n}{56}$. Finally, we show that $\tau(G)\leq \frac{3}{2}\nu(G)$ when $G$ is a complete 4-partite graph. Moreover, this bound is tight.

==> 4partitev2.tex <==
\section{Complete 4-Partite Graphs}
\label{section:tuza-complete-4partite}

Aparna \etal~\cite[Corollary 7]{Aparna11} showed that Tuza's Conjecture holds for
4-partite graphs.
In this section, we improve this bound for complete 4-partite graphs (Theorem \ref{theorem:tuza-4-partite-complete}).
We begin by stating a well-known theorem of Vizing.



We say that two edge colorings
$\{M_1, M_2, \ldots, M_k\}$ and
$\{N_1, N_2, \ldots, N_k\}$ of a graph $G$ are
\textit{compatible} 
if $|M_i \cap N_j| \leq 1$ for every $i,j$

\begin{lemma}
Any complete bipartie graph $G$ has two compatible edge colorings with size $\Delta(G)$.
\end{lemma}
\begin{proof}
Let $G=(B,C,E(G))$ be a complete bipartite graph with $|B|>|C|$.
Let $\mathcal{M}$ be an edge coloring of $G$.
We will show that there exists a compatible edge coloring with $\mathcal{M}$.
We proceed by induction on $|C|$.
If $|C|=1$, then the proof follows, as $\mathcal{M}$ is compatible with itself.
Now, suppose $|C|=2$. Let $u$ be an arbitrary vertex of $C$, and let $G'=(B,C-u,E(G'))$.
Let $\mathcal{M'} = \{M'_1, M'_2, \ldots, M'_b\}$,
where $M'_i = M_i \setminus \{vu \in E(G)\}$.

By induction hypothesis, there exists an edge coloring
$\mathcal{N'}$ compatible with $\mathcal{M'}$.
Let $\mathcal{N'}=\{N'_1, N'_2, \ldots, N'_b\}$.
Let $H = (\mathcal{M},\mathcal{N'}, E(H))$ be a bipartite
graph such that $M_iN'_j \in E(H)$ if and only if
$M_i \cap N'_j=\emptyset$.
As $|B|\geq |C|$, $d_H(M_i) = |\{N'_j: M_i \cap N'_j = \emptyset\}| =
|\{N'_j: M'_i \cap N'_j = \emptyset\}| =
|B|-|\{N'_j: M'_i \cap N'_j \neq \emptyset\}| =
|B|-|M'_i|= |B|-|C|+1$.
for every $i$. 
Also 
$d_H(N'_j) = |\{M_i: M_i \cap N'_j = \emptyset\}| =
|\{M'_i: M'_i \cap N'_j = \emptyset\}|=
|B|-|\{M'_j: M'_i \cap N'_j \neq \emptyset\}| =
|B|-|N'_i|= |B|-|C|+1$.
As $|B|\geq |C|$, $H$ is a regular bipartite graph
and thus has a perfect matching, say $F$.


For every $M_i \in \mathcal{M}$, 
let $f(M_i)$ be such that $M_if(M_i) \in F$.  
let $e_i$ be the edge in $M_i$ incident to $u$.
Let $N_i = f(M_i) \cup \{e_i\}$.
We will prove that $\mathcal{N}=N_1, \ldots, N_b$
is a matching compatible with $\mathcal{M}$.
Let $M_i \in \mathcal{M}, N_j \in \mathcal{N}$.
If $N_j = f(M_i)$, then $M_i \cap N_j = (\{e\}) $





\end{proof}


The next lemma will help us to find a subgraph of a complete bipartite
graph that is almost regular.
Given a vertex~$v$ in a graph~$G$, we say that
$d_G(v) \sim \ell$ if~$d_G(v) \in \{ \floor{\ell}, \ceil{\ell} \}$.

%last
\begin{lemma}\label{lemma:tuza-4partite-bipartido-balanceado}
Let~$G=(X,Y,E)$ be a complete bipartite graph 
with~$x=|X|$, $y=|Y|$ and ${x \geq y}$.
Let~$k$ be a positive integer with~${k \leq x}$.
There exists a subgraph $G'$ of~$G$, with the same vertex set of~$G$, such that
${d_{G'}(v) = k}$ for every~$v \in Y$
and~$d_{G'}(v) \sim yk/x$ for every~$v \in X$.
\end{lemma}
\begin{proof}
Let~$r= yk \mod x$.
Let~$X=\{v_0, v_1, \ldots, v_{x-1}\}$ and
$Y=\{w_0, w_1, \ldots, w_{y-1}\}$.
We construct a capacited directed graph~$D=(N,A,c)$
such that~$N= X \cup Y \cup \{s,t\}$,
and~$A= \{v_iw_j: v_i \in X, w_j \in Y\} \cup \{sv_i: v_i\in X\} \cup \{w_jt:w_j \in Y\}$,
$c(v_iw_j)=1$ if~${v_iw_j \in E(G)}$,
$c(sv_i)=\ceil{yk/x}$ if $i<r$,
$c(sv_i)=\floor{yk/x}$ if $i\geq r$,
and~$c(w_jt)=k$ for every~$w_j \in Y$.
We prove that every~$st$-cut has capacity at least~$ky$.
Let~$S$ be a set of nodes of~$D$ that separates~$s$ from~$t$.
%Then~$c(S)\geq \floor{yk/k}|X \setminus S| + |S \cap X| \cdot |Y \setminus S| + k|S \cap Y|$.
If~$|X \cap S| \geq k$, then
$c(S) \geq  k|Y \setminus S| + k|S \cap Y|= k|Y|$ and we are done.
So, suppose that~$|X \cap S| < k$. Then,
\begin{eqnarray*}
c(S)&=& \sum_{v_i \in X \setminus S}c(sv_i) + |X \cap S| \cdot |Y \setminus S| + k|Y \cap S| \\
      &=& \sum_{v_i \in X}c(sv_i) - \sum_{v_i \in X \cap S}c(sv_i) + |X \cap S| \cdot |Y \setminus S| + k|Y \cap S| \\
      &=& ky  - \sum_{v_i \in X \cap S}c(sv_i) + |X \cap S| \cdot |Y \setminus S| + k|Y \cap S| \\
      &>& ky  - \sum_{v_i \in X \cap S}\ceil{yk/x} + |X \cap S| \cdot |Y \setminus S| +  |X \cap S||Y \cap S| \\
      &=& ky  - |X \cap S|\ceil{yk/x} + |X \cap S| \cdot |Y|\\
      &=&ky  +  |X \cap S|(y-\ceil{yk/x}) \\
      &\geq& ky.
\end{eqnarray*} 

As there exists a cut of value~$ky$, by the max-flow min-cut theorem \cite{Ford56},
there exists a flow of value~$ky$.
By Dantzig and Fulkerson \cite{Dantzig55}, this flow is integer.
We can convert this flow into the desired subgraph.
\end{proof}

The next proposition shows how to convert edge-colorings in tripartite graphs
into packings in 4-partite graphs. It can be viewed as a generalization of
Proposition \ref{prop:prop2}.

\begin{proposition} \label{prop:tuza-4partite-ABCD}
Let~$G=(A,B,C,D,E(G))$ be a complete
4-partite graph.
If there exists a subgraph~$G'$ of~$G[B \cup C \cup D]$
with~$d_{G'}(v) \leq |A|-1$ for all~$v \in V(G')$, then~$\nu(G)  \geq |E(G')|$.
\end{proposition}
\begin{proof}
By Proposition~\ref{prop:tuza-vizing}, there exists an edge-coloring of $G'$
with cardinality at most~$a'\leq |A|$.
Let~$\{M_1, M_2,\ldots, M_{a'}\}$ be such a coloring. We can extend each of these matchings to form a packing of~$G$ in the following way.
Let~$\{v_1,v_2,\ldots,v_{a'}\} \subseteq A$.
For every~$i \in \{1,2,\ldots,a'\}$, let~$Y_i=\{v_iuw: uw \in M_i\}$.
Observe that every~$Y_i$ is a packing in~$G$, as every~$M_i$ is a matching in~$G'$.
Observe also that~$|Y_i|=|M_i|$. Also, as every pair of matchings
in~$\{M_1, M_2, \ldots , M_{a'}\}$ is disjoint, and each matching forms triangles with a different vertex from~$A$,
$Y=Y_1 \cup Y_2 \cup \cdots \cup Y_{a'}$ is a packing in~$G$ of cardinality
${|M_1| + |M_2| + \cdots + |M_{a'}| = |E(G')|}$.
\end{proof}

Finally, we prove the main theorem of this section.

\begin{theorem}\label{theorem:tuza-4-partite-complete}
%For every complete 4-partite graph~$G$,
Let~$G=(A,B,C,D,E(G))$ be a complete
4-partite graph with~$a:=|A|  \geq b:=|B|\geq c:=|C| \geq d :=|D|$, and $a>1$.
%${\tau(G) \leq \frac{2ad+2bc}{2ad+ac-2c-2d} \cdot \nu(G)}$.
\begin{itemize}
\item If~$a\geq b+c+1$, then~$\tau(G)=\nu(G)$.
\item If~$c+d < a \leq b+c$, then~$\tau(G) \leq \frac{ad+bc}{ad+bc-d} \cdot \nu(G)$.
\item If~$a \leq c+d$, then~${\tau(G)\leq \frac{2ad+2bc}{2ad+ac-2c-2d} \cdot \nu(G)}$.
\end{itemize}
\end{theorem}
\begin{proof}
%Let~$G=(A,B,C,D)$ be a complete
%4-partite graph with~$a:=|A|,b:=|B|, c:=|C|, d:=|D|$
%and~$a  \geq b \geq c \geq d$.
For every~$P$, $Q \in \{A,B,C,D\}$, we say that 
the~$PQ$ edges are the edges of~$G$ with one end
in~$P$ and the other in~$Q$.
We divide the proof in the three obvious cases.

 \setcounter{case}{0}
 
\begin{case}~$a\geq b+c+1$.

By Proposition \ref{prop:tuza-4partite-ABCD}, with~$G'=G[B \cup C \cup D]$,~$\nu(G)\geq bc+cd+bd$.
Also, the set of~$BC$ edges joined
to the set of~$CD$ and~$BD$ edges form a hitting set of~$G$,
with cardinality~$bc+cd+bd$.
Thus
$\tau(G)\leq  bc+cd+bd  \leq \nu(G).$

\end{case}

\begin{case}~$c+d < a \leq b+c$.

By Lemma~\ref{lemma:tuza-4partite-bipartido-balanceado}, 
with~$k=a-b-1\leq c$, there exists a subgraph~$G'_{CD}$ of
$G[C \cup D]$ such that~$d_{G'_{CD}}(v) = a-b-1$ for every~$v \in D$
and~$d_{G'_{CD}}(v) \sim \frac{d}{c}(a-b-1) \leq a-b-1$ for every~$v \in C$.
Let~$G'=G[B \cup D] \cup G[B \cup C] \cup G'_{CD}$.
Observe that, for every~$v \in V(G')$, we have~$d_{G'}(v) \leq a-1$.
Indeed, if~$v\in B$, then~$d_{G'}(v)=c+d \leq a - 1$;
if~$v\in C$, then~$d_{G'}(v) \leq b+(a-b-1) = a - 1$;
if~$v\in D$, then~$d_{G'}(v) = b + (a-b-1) = a-1$.
By Proposition \ref{prop:tuza-4partite-ABCD},
$\nu(G) \geq |E(G')|=bc+bd+(a-b-1)d=bc+ad-d$.
Also, the set of~$BC$ edges joined
to the set of~$AD$ edges form a hitting set of~$G$,
with cardinality~$ad+bc$.
Hence, 
$\tau(G)\leq ad+bc \leq \frac{ad+bc}{ad+bc-d} \, \nu(G).$
\end{case}

\begin{case}~$a \leq c+d$.

By Lemma~\ref{lemma:tuza-4partite-bipartido-balanceado},
with~${k=\floor{\frac{a-1}{2}} \leq c}$, there exists a subgraph~$G'_{CD}$ of
$G[C \cup D]$ such that~${d_{G'_{CD}}(v) = \floor{\frac{a-1}{2}}}$ for every~$v \in D$,
and~${d_{G'_{CD}}(v) \sim \frac{d}{c}(\floor{\frac{a-1}{2}}) \leq \floor{\frac{a-1}{2}}}$ for every~$v \in C$.
By Lemma~\ref{lemma:tuza-4partite-bipartido-balanceado},
with~${k=\ceil{\frac{a-1}{2}} \leq b}$, there exists a subgraph~$G'_{BD}$ of
$G[B \cup D]$ such that~${d_{G'_{BD}}(v) = \ceil{\frac{a-1}{2}}}$ for every~$v \in D$,
and~${d_{G'_{CD}}(v) \sim \frac{d}{b}(\ceil{\frac{a-1}{2}}) \leq \ceil{\frac{a-1}{2}}}$ for every~$v \in B$.
By Lemma~\ref{lemma:tuza-4partite-bipartido-balanceado},
with~$k=\floor{\frac{a-1}{2}} \leq b$, there exists a subgraph~$G'_{BC}$ of
$G[B\cup C]$ such that~$d_{G'_{BC}}(v) = \floor{\frac{a-1}{2}}$ for every~$v \in C$,
and~$d_{G'_{BC}}(v) \sim \frac{b}{c}(\floor{\frac{a-1}{2}}) \leq \floor{\frac{a-1}{2}}$ for every~$v \in B$.
Let~$G'=G'_{BD} \cup G'_{BC} \cup G'_{CD}$.

Observe that, for every~$v \in V(G')$, we have~$d_{G'}(v) \leq a-1$.
Indeed, if~$v\in B$, then~$d_{G'}(v)=d_{G'_{BC}}(v)+d_{G'_{BD}}(v)  \leq \floor{\frac{a-1}{2}} +  \ceil{\frac{a-1}{2}} = a-1$;
if~$v\in C$, then~$d_{G'}(v) = d_{G'_{BC}}(v)+d_{G'_{CD}}(v)  \leq 2\floor{\frac{a-1}{2}} \leq a - 1$;
if~$v\in D$, then~$d_{G'}(v) = d_{G'_{BD}}(v)+d_{G'_{CD}}(v) = \floor{\frac{a-1}{2}} +  \ceil{\frac{a-1}{2}} = a-1$.
Thus,
by Proposition \ref{prop:tuza-4partite-ABCD},
\begin{eqnarray*}
\nu(G) &\geq& |E(G')| \\
&=& |E(G'_{BC})|+|E(G'_{CD})|+|E(G'_{BD})| \\
&=& c \Floor{\frac{a-1}{2}} + d \Floor{\frac{a-1}{2}} + d \Ceil{\frac{a-1}{2}}  \\
&=& c \Floor{\frac{a-1}{2}} + d(a-1) \\
&\geq& c(\frac{a}{2}-1) + d(a-1) \\
&=& ad+\frac{ac}{2}-c-d.
\end{eqnarray*}
Also, the set of~$BC$ edges joined
to the set of~$AD$ edges form a hitting set of~$G$,
with cardinality~$ad+bc$.
Hence, as $a>1$,
$\tau(G)\leq  ad+bc  \leq \frac{2ad+2bc}{2ad+ac-2c-2d} \cdot \nu(G).$
\end{case}
This concludes the proof of the theorem.
\end{proof}

As we see in the next corollary, Theorem \ref{theorem:tuza-4-partite-complete} improves
the result of Aparna et al in cases 1 and 2.

\begin{corollary}
Let~$G=(A,B,C,D,E(G))$ be a complete
4-partite graph with~$a:=|A|  \geq b:=|B|\geq c:=|C| \geq d :=|D|$. If $a>c+d$ then $\tau(G) \leq \frac{3}{2}\nu(G)$.
\end{corollary}

==> split.tex <==
In this section, we will show that Tuza's conjecture
holds for split graphs with minimum degree at least
$0.57n$. In fact, we will prove the next stronger result.

\begin{theorem}\label{teorema:dense-split}
    Let~$G=(K,S,E(G))$ be a split graph on~$n$ vertices. Then Conjecture \ref{conjecture:tuza} holds when at least one of the following conditions is satisfied:
    \begin{itemize}
        \item~$\delta(G) \geq \frac{1}{2} + \sqrt{\frac{n^2 -2n +2}{8}}$ and~$|S| \geq |K|$,
        \item~$\delta(G) \geq \frac{n+2}{4} + \sqrt{\frac{5n^2 + 26n - 72}{48}}$ and~$|S| < |K|$, or
        \item 5$|S| \leq |K|$ and~$n \geq 57$.
    \end{itemize}

\end{theorem}

We begin by state two known results for the size of a maximum packing when the graph is a complete split graph, and a complete graph.

\begin{proposition}[{\cite[see
Corollary 5]{Bonamy2021}}]\label{prop:prop3}
For every complete split graph~$G=(K,S,E(G))$, there exists a packing in which all triangles have vertices in~$K$ and in~$S$, with size~$\frac{| K | - 1}{2} \cdot \min\{| S |, | K |\}$.
\end{proposition}

 \begin{proposition}[{\cite[
Theorem 2]{Feder2012}}]
\label{prop:pK}
%If~$n\geq6$, then~$|p(K_n)|\geq \frac{1}{3}({{n}\choose{2}} - \frac{n}{2} - 1 ).$
For every $n \geq 2$, we have
$\nu(K_n)=\frac{1}{3}({{n}\choose{2}} - k)$, where
%$k = 0$ if~$n$ MOD 6~$\in \{1,3\}$,
%$k=4$ if~$n$ MOD 6 =5,
%$k=\frac{n}{2}$ if~$n$ MOD 6 =$\in \{0,2\}$, and
%$k=\frac{n}{2} + 1$ if $n$ MOD 6 =4.
$$
k=
\begin{cases}
0 & \text{: }n \text{ MOD } 6 \in \{1,3\}\\
4 & \text{: }n \text{ MOD } 6 =5\\
 \frac{n}{2} & \text{: }n \text{ MOD } 6 \in \{0,2\}\\
\frac{n}{2} + 1 & \text{: } n \text{ MOD } 6 =4.
\end{cases}
$$
%\end{equation*}
Thus,~$\nu(K_n) \geq \frac{1}{3}({{n}\choose{2}} - \frac{n}{2} - \frac{3}{2})$ for every~$n \geq 2$. 
\end{proposition}


We now apply our Lemma \ref{lemma:main} to the case of split graphs, and obtain the next two corollaries.

\begin{corollary}[see also {\cite[
Proposition 4]{Gyori87}}] \label{cor:nu(G)geqTGnu(K_n)n3}
For any graph~$G$ of~$n$ vertices,~$\nu(G)~\geq~\frac{|\mathcal{T}(G)|\times \nu(K_n)}{\binom{n}{3}}$.
\end{corollary}
\begin{proof}
Let~$G'=K_n$, let~$\Pi^{'} = \mathfrak{S}(G')$ and let~$P'$ be a maximum packing in~$G'$. Note that, for a fixed~$(t,t') \in \mathcal{T}(G)  \times P'$, there are exactly~$6(n-3)!$ permutations~$\pi \in \Pi^{'}$ such that~$t = \pi(t')$. Then, by Lemma \ref{lemma:main}, we have~$\nu(G)~\geq~ \frac{|\mathcal{T}(G)|\times |P'| \times 6(n-3)!}{n!} = \frac{|\mathcal{T}(G)|\times \nu(K_n)}{\binom{n}{3}}$.
\end{proof}

\begin{corollary} \label{cor:corollary2}
Let~$G=(K,S,E(G))$ be a split graph on~$n$ vertices, then~$\nu(G) \geq \frac{|T'|}{\max(|S|,|K|)}$, where~$T'$ is the set of triangles in~$G$ with vertices in~$K$ and~in~$S$. 
\end{corollary}
\begin{proof}
Let~$G' = (K,S,E(G'))$ be a complete split graph and let~$\Pi^{'} \subseteq \mathfrak{S}(G')$ be such that, for each~$\pi \in \Pi^{'}$,~$\pi(v) 
 \in V(K)$ if and only if~$v \in V(K)$. Note that, by Proposition \ref{prop:prop3}, there exists a packing~$P^{'}$ in~$G'$, in which all triangles have vertices in~$K$ and in~$S$, with size at least~$\frac{|K|-1}{2} \cdot \min(|S|,|K|)$. Also, for a fixed~$(t,t') \in T' \times P'$, there are exactly~$2(|K|-2)!\times (|S|-1)!$ permutations~$\pi \in \Pi^{'}$ such that~$t = \pi(t')$. Thus, by Lemma \ref{lemma:main}, we have~$\nu(G) \geq \frac{|T'|\times|P'|\times 2(|K|-2)!\times (|S|-1)!}{|K|! \times |S|!} = \frac{|T'| \times |P'|}{|S| \times \binom{|K|}{2}} \geq \frac{|T'|}{\max(|S|,|K|)}$.
 \end{proof}

We now proceed to the proof of Theorem \ref{teorema:dense-split}. We will consider three cases based on the conditions of Theorem \ref{teorema:dense-split}.
Also, as Conjecture \ref{conjecture:tuza} is valid when~$n \leq$ 4 \cite[Theorem 1.2]{Puleo15}, we will assume that~$n\geq 5$.

\begin{case}
$\delta(G) \geq \frac{1}{2} + \sqrt{\frac{n^2 -2n +2}{8}}$ and~$|S| \geq |K|$.
\end{case}
By the case condition, we have that
$\delta^2(G) - \delta(G) \geq \frac{n(n-2)}{8}$.
Note that~$\nu(G) \geq \sum_{u \in S} \binom{d(u)}{2}/|S|$, by Corollary \ref{cor:corollary2}. Also,~$\tau(G) \leq \binom{|K|}{2}$, because the set of all edges in~$K$ is a hitting set of~$G$. Then, as~$|K| \leq \frac{n}{2}$, \begin{eqnarray} \tau(G) \leq \binom{|K|}{2} \leq \frac{n^2 -2n}{8} \leq  \delta^2(G) - \delta(G). \label{eq:e} \end{eqnarray}
Also, by Cauchy-Schwarz inequality,~$\sum_{u \in S} d^2(u) \geq (\sum_{u \in S} d(u))^2/|S|$. Hence, 
\begin{eqnarray}
2\nu(G)
 &\geq& \frac{1}{|S|}\Big(\sum_{u \in S} d^2(u) - \sum_{u \in S} d(u)\Big) \nonumber \\
 &\geq& \frac{1}{|S|^2}\Big((\sum_{u \in S} d(u))^2 - |S|\sum_{u \in S} d(u)\Big) \nonumber \\
 &\geq&  \delta^2(G) - \delta(G). \label{eq:2}
\end{eqnarray}
By \eqref{eq:e} and \eqref{eq:2}, we have ~$2\nu(G) \geq \tau(G)$, as we want. This finishes the proof of Case 1.\\

Let~$k = |K|$. By Proposition \ref{prop:pK},~$\nu(K_n) \geq \frac{n^2 -2n -3}{6}$. Thus, as~$n \geq 5$, we have~$\nu(K_n) \geq \frac{(n-2)(n-1)}{6}$. Also, by Corollary \ref{cor:nu(G)geqTGnu(K_n)n3}, we have that~$\nu(G) \geq \Big(\binom{k}{3} + \sum_{u \in S} \binom{d(u)}{2}\Big) \cdot  \nu(K_n)/\binom{n}{3} \geq \Big(\binom{k}{3} + \sum_{u \in S} \binom{d(u)}{2}\Big)/n$. As~$G$ has a hitting set with size at most~$|E(G)|/2$, we have~$\tau(G) \leq \frac{1}{2}(\binom{k}{2} + \sum_{u \in S} d(u))$. Hence, by Cauchy-Schwarz inequality, we have that
\begin{eqnarray}
2\nu(G) - \tau(G) 
&\geq& \frac{1}{12n}\Big(24\binom{k}{3} + 12\sum_{u \in S} d^2(u) - 12\sum_{u \in S} d(u) -6n\binom{k}{2} -6n\sum_{u \in S} d(u)\Big) \nonumber \\
&\geq &
\frac{1}{n}\Big((\sum_{u \in S} d(u))^2/|S|\Big)  - \frac{n+2}{2n}\sum_{u \in S} d(u) 
+\frac{2}{n}\binom{k}{3}-\frac{1}{2}\binom{k}{2}
\nonumber
\\ 
&=&
\frac{1}{n}\Big((\sum_{u \in S} d(u))^2/|S|\Big)  - \frac{n+2}{2n}\sum_{u \in S} d(u) + \frac{1}{12n}\Big(k(k-1)(4k-3n-8)\Big).
\label{eq:4}
\end{eqnarray}
\begin{case}
$\delta(G) \geq \frac{n+2}{4} + \sqrt{\frac{5n^2 + 26n - 72}{48}}$ and~$|S| < |K|$.
\end{case}
%By the case condition, we have that
%$\delta^2(G) - \delta(G)(\frac{n+2}{2}) - \frac{n^2 +7n -42}{24} \geq 0$. 
%Also, 
By \eqref{eq:4}, we have
\begin{eqnarray}
2\nu(G) - \tau(G)
%&\geq& 
%\frac{1}{n}\Big(\delta^2(G)(n-k) - \delta(G)(n-k)(n+2)/2 + 2\binom{k}{3}  - \frac{n}{2}\binom{k}{2}\Big) \nonumber \\ 
%&=& 
%\frac{n-k}{n}
%\Big( 
%\delta^2(G) - \delta(G)(n+2)/2 + \frac{2}{n-k}\binom{k}{3} - \frac{n}{2(n-k)}\binom{k}{2} \Big) \nonumber \\
&\geq&
\frac{n-k}{n}
\Big( 
\delta^2(G) - \delta(G)(n+2)/2 + \frac{k(k-1)}{n-k} \cdot \frac{4k-3n-8}{12} \Big) \nonumber \\
&\geq&
\frac{n-k}{n}
\Big( 
\delta^2(G) - \delta(G)(n+2)/2 + k \cdot \frac{4k-3n-8}{12} \Big) \nonumber \\
&\geq&
\frac{n-k}{n}\Big(\delta^2(G) - \delta(G)(n+2)/2 - (n^2 +7n +6)/24\Big) \nonumber
\\
  &\geq& \frac{n-k}{n} \cdot (-2) \nonumber \\
  &>& -1 \nonumber
\label{eq:5}.
\end{eqnarray}
Where the third inequality is valid
because~$k \cdot \frac{4k-3n-8}{12}$ is an increasing function on $k$ and~$k \geq \frac{n+1}{2}$, and the fourth inequality is valid by the case condition.
%\begin{eqnarray}
%2\nu(G) - \tau(G)
% &\geq&
% \frac{n-k}{n}\Big(\delta^2(G) - \delta(G)(n+2)/2 - (n^2 +7n +6)/24\Big) \nonumber \\
%  &\geq& \frac{n-k}{n} \cdot (-2) \nonumber \\
%  &>& -1. \nonumber
%\end{eqnarray}
Since~$2\nu(G) - \tau(G)$ is integer, we have~$2\nu(G) - \tau(G) \geq 0$. This finishes the proof of Case 2.
\begin{case}
5$|S| \leq |K|$ and~$n \geq 57$.
\end{case}
By \eqref{eq:4}, we have
\begin{eqnarray}
2\nu(G) - \tau(G)  
&\geq&
\frac{1}{n(n-k)}(\sum_{u \in S} d(u))^2 - \frac{n+2}{2n}\sum_{u \in S} d(u) + \frac{1}{12n}\Big(k(k-1)(4k-3n-8)\Big) \nonumber \\
&>& \frac{1}{n(n-k)}(\sum_{u \in S} d(u))^2 - \frac{n+2}{2n}\sum_{u \in S} d(u) + \frac{1}{12n}\Big(k(k-1)(4k-3n-8)+12n-1\Big) - 1 \nonumber \\
&\geq& \frac{6}{n^2}\Big(\sum_{u \in S} d(u)\Big)^2 - \frac{n+2}{2n}\sum_{u \in S} d(u) +\frac{1}{1296n}\Big(5n(5n-6)(n-24) + 108(12n-1)\Big) -1 \nonumber \\
&=& \frac{6}{n^2}\Big((\sum_{u \in S} d(u))^2 - \frac{n(n+2)}{12}\sum_{u \in S} d(u) + \frac{(5n^2(5n-6)(n-24) + 108n(12n-1))}{7776}\Big) - 1 \nonumber \\ 
&\geq& -1 \nonumber,
\end{eqnarray}
where the third inequality is valid 
because~$k \geq \frac{5n}{6}$, 
and the last inequality is valid because~$\frac{5n^2(5n-6)(n-24) + 108n(12n-1)}{7776} \geq (\frac{n(n+2)}{24})^2$ for~$n \geq 57$. Since~$2\nu(G) - \tau(G)$ is integer, we have~$2\nu(G) - \tau(G) \geq 0$.






















































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































